Correlation-Attention Masked Temporal Transformer for User Identity Linkage Using Heterogeneous Mobility Data

With the rise of social media and Location-Based Social Networks (LBSN), check-in data across platforms has become crucial for User Identity Linkage (UIL). These data not only reveal users' spatio-temporal information but also provide insights into their behavior patterns and interests. However, cross-platform identity linkage faces challenges like poor data quality, high sparsity, and noise interference, which hinder existing methods from extracting cross-platform user information. To address these issues, we propose a Correlation-Attention Masked Transformer for User Identity Linkage Network (MT-Link), a transformer-based framework to enhance model performance by learning spatio-temporal co-occurrence patterns of cross-platform users. Our model effectively captures spatio-temporal co-occurrence in cross-platform user check-in sequences. It employs a correlation attention mechanism to detect the spatio-temporal co-occurrence between user check-in sequences. Guided by attention weight maps, the model focuses on co-occurrence points while filtering out noise, ultimately improving classification performance. Experimental results show that our model significantly outperforms state-of-the-art baselines by 12.92%~17.76% and 5.80%~8.38% improvements in terms of Macro-F1 and Area Under Curve (AUC).

==> 7checklist.tex <==
% Checklist macros
% \clearpage
\newcommand{\answerYes}[1]{\textcolor{blue}{#1}} 
\newcommand{\answerNo}[1]{\textcolor{yellow}{#1}} 
\newcommand{\answerNA}[1]{\textcolor{gray}{#1}} 
\newcommand{\answerPartial}[1]{\textcolor{green}{#1}}
\newcommand{\answerTODO}[1]{\textcolor{red}{#1}} 

\section{Reproducibility checklist}

Unless specified otherwise, please answer [Yes] to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled ``Reproducibility Checklist'' at the end of the technical appendix.

\noindent This paper:

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. \answerYes{Yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. \answerYes{Yes}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper.  \answerYes{Yes}
\end{itemize}

\noindent Does this paper make theoretical contributions?  \answerYes{Yes}

\noindent If yes, please complete the list below.

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no) \answerYes{Yes}
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no) \answerYes{Yes}
    \item Proofs of all novel claims are included. (yes/partial/no) \answerYes{Yes}
    \item Proof sketches or intuitions are given for complex and/or novel results.  (yes/partial/no) \answerYes{Yes}
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no) \answerYes{Yes}
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA) \answerYes{Yes}
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA) \answerYes{Yes}
\end{itemize}

\noindent Does this paper rely on one or more datasets? (yes/no) \answerYes{Yes}

\noindent If yes, please complete the list below.

\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets. (yes/partial/no/NA) \answerYes{Yes}
\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) \answerYes{Yes}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) \answerYes{Yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) \answerYes{Yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) \answerYes{Yes}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) \answerYes{Yes}
\end{itemize}


\noindent Does this paper include computational experiments? (yes/no)
\answerYes{Yes}

\noindent If yes, please complete the list below.
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes/partial/no) \answerYes{Yes}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) \answerYes{Yes}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) \answerYes{Yes}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) \answerYes{Yes}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) \answerYes{Yes}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) \answerYes{Yes}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) \answerYes{Yes}
\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) \answerYes{Yes}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) \answerYes{Yes}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) \answerYes{Yes}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) \answerYes{Yes}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) \answerYes{Yes}
\end{itemize}

==> table/notations.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{c|c}
\hline
\textbf{Notation} & \textbf{Definition} \\ \hline
${\cal U}_A$   & user sets of platform A \\ 
${\cal U}_B$ & user sets of platform B \\
$u_i$ & a user \\
$t$   & the timestamp of the check-in \\ 
$p$ & a POI \\
${\cal T}_{u_i}$ & the check-in sequence of $u_i$ \\
$\cal P$ & the POI sets of $p$ \\
$T$ & the time slot sets of $t$ \\
$f_\theta(\cdot)$ & a mapping function of \model \\
${{\bf{E}}_p}$ & the embeddings of each $p$ \\
${{\bf{E}}_t}$ & the embeddings of each time slot of $t$ \\
$x$ & the joint embeddings of ${{\bf{E}}_p}$ and ${{\bf{E}}_t}$\\
${\bf{X}}$ & the embeddings of check-in sequences \\
$f_{st}(\cdot)$ & the spatial-temporal embedding layer \\
${\bf{z}}$ & the spatial-temporal embedding of $x$ \\
${\bf{Z}}$ & the spatial-temporal embeddings of ${\bf{z}}$ \\
${f_{\rm T}}(\cdot)$ & the temporal transformer encoder \\
${\bf{H}}$ & the spatio-temporal representation \\
${\bf{Q}}$ & the query vector of ${\bf{H}}$ \\
${\bf{K}}$ & the key vector of ${\bf{H}}$ \\
${\bf{V}}$ & the value vector of ${\bf{H}}$ \\
$H$ & number of heads for multi-head attention \\
$h$ & the $h$-th attention head \\
${\bf{Attn}}$ & the attention weight map \\
${f_{\rm M}}(\cdot)$ & the masked transformer encoder \\
${{\bf{I}}}$ & the index vector of attention weight map \\
${\bf{H}}^m$ & the representation of masked transformer \\
${{\bf{M}}_{mask}}$ & the mask matrix \\
\hline
\end{tabular}
\caption{Summary of key notations.}
\label{tab:notations}
\end{table}

==> table/parameters.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{c|cc}
\hline
\textbf{Hyperparameters} & $f_{\rm M}$ & $f_{\rm T}$ \\ \hline
POI embedding dimension         & 64 & 64 \\ 
time embedding dimension        & 16 & 16 \\ 
check-in embedding dimension    & 64 & 64 \\ 
Layers                          & 4 & 4 \\ 
FFN inner hidden size           & 128 & 128 \\ 
Attention heads                 & 8 & 8 \\ 
Attention head size             & 8  & 8 \\ 
\midrule
Training epochs                 & \multicolumn{2}{c}{50} \\ 
Batch size                      & \multicolumn{2}{c}{32} \\ 
Initial learning rate           & \multicolumn{2}{c}{1e-3} \\ 
Learning rate schedule          & \multicolumn{2}{c}{multiplicative (5, 0.9)} \\ 
Dropout                         & \multicolumn{2}{c}{0.1} \\ 
\midrule
mask ratio                       & \multicolumn{2}{c}{0.15} \\ 
\hline
\end{tabular}
\caption{Hyperparameters for $f_{\rm M}$ and $f_{\rm T}$ models.}
\label{tab:parameters}
\end{table}
